Holder Continuous Solutions of Active Scalar Equations

We consider active scalar equations $\partial_t \theta + \nabla \cdot (u \, \theta) = 0$, where $u = T[\theta]$ is a divergence-free velocity field, and $T$ is a Fourier multiplier operator with symbol $m$. We prove that when $m$ is not an odd function of frequency, there are nontrivial, compactly supported solutions weak solutions, with H\"older regularity $C^{1/9-}_{t,x}$. In fact, every integral conserving scalar field can be approximated in ${\cal D}'$ by such solutions, and these weak solutions may be obtained from arbitrary initial data. We also show that when the multiplier $m$ is odd, weak limits of solutions are solutions, so that the $h$-principle for odd active scalars may not be expected.

==> theConstruction.tex <==
We now give a detailed description of the construction.  We start by obtaining a complete list of the error terms.

Suppose that we are in the setting of Lemma \ref{lem:mainLemma}.  Thus, we have a solution $(\th, u, c_A, R_J)$ to the compound scalar-stress equation with vector $A^l = m^l(\xi^{(1)}) + m^l(-\xi^{(1)})$ as in \eqref{eq:ourAlandBl}
\ali{
\left \{
\begin{aligned}
\pr_t \th + \pr_l(\th u^l) &= \pr_l( c_A A^l + R_J^l)  \\
u^l &= T^l(\th) 
\end{aligned}
\right.
}
whose frequency-energy levels are below $(\Xi, e_v, e_R, e_J)$.  After adding a correction $\Th$ to the scalar field, the corrected scalar $\th_1 = \th + \Th$ and drift velocity $u_1^l = u^l + U^l$, $U^l = T^l[\Th]$ satisfy the system
\ali{
\pr_t \th_1 + \pr_l(\th_1 u_1^l) &= \pr_t \Th + \pr_l( u^l \Th) + \pr_l(\th U^l) + \pr_l( \Th U^l c_A A^l + R_J^l) \label{eq:correctedSystem1}
}
As a preliminary step, it is necessary to define suitable regularizations $(\th_\ep, u_\ep, \tilde{c}_A, R_\ep)$ of the given $(\th, u, c_A, R_J)$.  The purpose of these regularizations is to ensure that only the ``low frequency parts'' of the given solutions $(\th, u, c_A, R_J)$ will influence the building blocks of the construction.  These mollifications give rise to an error term
\ali{
R_M^l &= (u^l - u_\ep^l) \Th + (\th - \th_\ep)U^l + (c_A - \tilde{c}_A) A^l + (R_J^l - R_\ep^l) \label{eq:mollifyRappears}
}
Our goal is to design a correction $\Th$ for the scalar field $\th$ so that the corrected scalar $\th_1 = \th + \Th$ and drift velocity $u_1^l = u^l + U^l$ satisfy the compound scalar-stress equation with vector $B^l = m^l(\xi^{(2)}) + m^l(-\xi^{(2)})$ as in \eqref{eq:ourAlandBl}
\ali{
\label{eq:scalarStressB}
\left \{
\begin{aligned}
\pr_t \th_1 + \pr_l(\th_1 u_1^l) &= \pr_l( c_B B^l + R_1^l)  \\
u_1^l &= T^l[\th_1] 
\end{aligned}
\right.
}
whose compound frequency energy levels are bounded as in Lemma \ref{lem:mainLemma}.

%Our mollification parameters are chosen in terms of the frequency-energy levels $(\Xi, e_v, e_R, e_J)$ and the frequency growth parameter $N$ to achieve the estimate
%\ali{
%\co{ R_M } &\unlhd \fr{e_v^{1/2} e_R^{1/2}}{500 N}
%}
%Here the notation $\unlhd$ refers to an inequality which is a goal, but which remains to be proven.
\subsection{The shape of the corrections}\label{sec:shapeOfCorrections}
Our correction is a sum of individual waves
\ali{
\Th &= \sum_I \Th_I \\
\Th_I &= e^{i \la \xi_I}(\th_I + \de \th_I) \label{eq:aThILooksLike}
}
where we are free to specify the amplitudes $\th_I$ and the phase function $\xi_I$.  The parameter $\la$ is a large frequency parameter of the form
\ali{
\la &= B_\la N \Xi \label{eq:lambdaDef}
}
where $B_\la$ is a very large constant associated to $\la$ which is chosen at the end of the argument.  We require also that $\la \in \Z$ is an integer so that $e^{i \la \xi_I}$ is globally well-defined on the torus.  The term $\de \th_I$ in \eqref{eq:aThILooksLike} is a small correction term which is present to ensure that the wave $\Th_I$ has compact support in frequency space.  We will specify $\de \th_I$ later, but it is important to remark that 
\[ \co{\de \th_I} \to 0, \tx{ as } \la \to \infty \]
Each wave $\Th_I$ has a conjugate wave $\Th_{\bar{I}} = \overline{\Th}_I$ with an opposite phase function $\xi_{\bar{I}} = - \xi_I$ and amplitude $\th_{\bar{I}} = \bar{\th}_I$ so that the overall correction is real-valued.  We will choose the amplitudes $\th_I = \bar{\th}_I$ to be real-valued as well.

The index $I$ for the wave $\Th_I$ consists of two parts $I = (k,f) \in \Z \times \{ \pm \}$.  The discrete index $k \in \Z$ specifies the support of the wave $\Th_I = \Th_{(k,f)}$ in time.  Specifically, the support of $\Th_{(k,f)}$ will be contained in the time interval $[(k - \fr{2}{3}) \tau, (k + \fr{2}{3})\tau]$ where $\tau$ is a time scale parameter that will be chosen during the iteration.  The index $f \in \{ \pm \}$ is a sign which specifies the direction of oscillation of the wave $\Th_{(k,f)}$.  

The phase functions $\xi_I$ are solutions to the transport equation
\ali{
(\pr_t + u_\ep^l \pr_l) \xi_I &= 0 \label{eq:transportEqn}
}
The amplitudes $\th_I$ will be supported on a small time interval during which the phase functions remain close to their initial data.  The initial data for the phase function $\xi_I = \xi_{(k,f)}$ is chosen at the time $t(I) = k \tau$ depending on the sign $f = \pm$ of the index $I = (k,f)$
\ali{
\xi_I(t(I), x) = \xi_{(k, \pm)}(k \tau, x) &= \pm \xi^{(1)} \cdot x
}
Thus, there are two types of waves: $+$ waves $\Th_{(k,+)}$ which are indexed by $I = (k,+) \in \II_+ = \Z \times \{+\}$ and $-$ waves $\Th_{(k,-)}$ which are indexed by $I = (k,-) \in \II_- = \Z \times \{-\}$.  These waves are conjugate to each other and oscillate in essentially opposite directions
\ali{ 
\nab \xi_{(k, \pm)} &\approx \pm \xi^{(1)} 
}
We can therefore decompose the correction $\Th$ as
\ali{
\Th &= \Th_+ + \Th_- \\
\Th_{\pm} &= \sum_{I \in \II_\pm} \Th_I \\
\Th_- &= \bar{\Th}_+ 
}
Our individual waves are localized in frequency and take the form
\ali{
\Th_I &= P_{\approx \la}^\pm [ e^{i \la \xi_I} \th_I ] \label{eq:ThIisLike}
}
The operators $P_{\approx \la}^{\pm}$ in \eqref{eq:ThIisLike} restrict to frequencies of order $\la$ in a neighborhood of $\pm \la \xi^{(1)}$.  To be explicit, let ${\hat \eta}^{\pm}_{\approx 1}(\xi)$ be bump functions supported on frequencies 
\[ {\hat \eta}_{\approx 1}^{\pm}(\xi) \in C_c^\infty\left(B_{|\xi^{(1)}|/2}(\pm \xi^{(1)}) \right) \]
which are reflections of each other
\[ {\hat \eta}^-(\xi) = {\hat \eta}^+(-\xi) \]
and have the property that \[ {\hat \eta}^\pm_{\approx 1}(\xi) = 1, \qquad ~\tx{if } |\xi - (\pm \xi^{(1)})| \leq \fr{1}{4} |\xi^{(1)}| \] 
Set ${\hat \eta}^{\pm}_{\approx \la}(\xi) = {\hat \eta}^{\pm}_{\approx 1}(\la^{-1} \xi)$ to be a rescaling of ${\hat \eta}_{\approx 1}^\pm$ supported on high frequencies of order $\la$.  Then $P_{\approx \la}^{\pm}$ is given explicitly by a Fourier multiplier 
\[ \widehat{P_{\approx \la}^{\pm} F}(\xi) = {\hat \eta}_{\approx \la}^\pm(\xi) {\hat F}(\xi) \]   
Including this ``projection operator'' $P_{\approx \la}^{\pm}$ guarantees that all the corrections \eqref{eq:ThIisLike} have frequency support in the ball $| \xi - ( \pm \la \xi^{(1)} ) | \leq \la \fr{|\xi^{(1)}|}{2} $, and in particular have integral $0$.  Having compact support in the frequency space will allow us to easily control the resulting increment to the velocity field, which is obtained by applying another Fourier multiplier.

By the Microlocal Lemma \ref{lem:microlocal}, it is possible to write the wave \eqref{eq:ThIisLike} in the form \eqref{eq:aThILooksLike} with an explicit remainder $\de \th_I$, since we have
\ali{
P_{\approx \la}^\pm [ e^{i \la \xi_I} \th_I ] &= e^{i \la \xi_I}( \th_I {\hat \eta}_{\approx \la}^\pm(\la \nab \xi_I) + \de \th_I) \\
&= e^{i \la \xi_I}( \th_I + \de \th_I)
}
provided that the phase gradient is sufficiently close to its initial value
\ali{
| \nab \xi_I - (\pm \xi^{(1)}) | &\unlhd \fr{|\xi^{(1)}|}{4} \label{eq:keepPhaseGradientClose}
}
We will verify that inequality \eqref{eq:keepPhaseGradientClose} is satisfied when the parameter lifespan parameter $\tau$ is chosen.

Applying the Microlocal Lemma \ref{lem:microlocal} again, we can also calculate the resulting correction to the drift velocity.
\ali{
U_I^l := T^l \Th_I \\
T^l P_{\approx \la}^\pm [ e^{i \la \xi_I} \th_I ] &= e^{i \la \xi_I}(\th_I {\hat K}^l(\la \nab \xi_I) {\hat \eta}_{\approx \la}^\pm(\la \nab \xi_I) + \de u_I^l ) \\ 
&= e^{i \la \xi_I}( \th_I m^l(\nab \xi_I) + \de u_I^l )
}
Therefore, once we have verified \eqref{eq:keepPhaseGradientClose}, we have
\ali{
U_I^l &= e^{i \la \xi_I}( u_I^l + \de u_I^l) \\
u_I^l &= \th_I m^l(\nab \xi_I) \label{eq:uIexpression}
}
with an explicit error term $\de u_I^l$ given by Lemma \ref{lem:microlocal}.  We also obtain a decomposition of the drift velocity into $+$ and $-$ parts
\[ U^l = U_+^l + U_-^l, \qquad U_{\pm}^l = T^l[\Th_\pm] \]

\subsection{ Choosing the amplitudes }\label{sec:chooseAmplitudes}
According to Section \ref{sec:shapeOfCorrections}, we can now decompose the remaining error terms in Equation \eqref{eq:correctedSystem1} using the $\pm$ decomposition of $\Th = \Th_+ + \Th_-$ and $U^l = U_+^l + U_-^l$
\ali{
\pr_t \th_1 + \pr_l(\th_1 u_1^l) &= \pr_t \Th + \pr_l( u_\ep^l \Th) + \pr_l(\th_\ep U^l) \label{eq:transAndHighLow}\\
&+ \pr_l( \Th_- U_+^l + \Th_+ U_-^l + \tilde{c}_A A^l + R_\ep^l) \label{eq:theStressTerm} \\
&+ \pr_l(\Th_- U_-^l + \Th_+ U_+^l) \label{eq:highFreqTerms} \\
&+ \pr_l R_M^l
}
The term $R_M^l$ comes from the regularizations in Equation \eqref{eq:mollifyRappears}.

The first objective of the correction is to eliminate the term \eqref{eq:theStressTerm}, which is the only low frequency term that arises.  However, since we consider oscillations in essentially only one direction $\nab \xi_I \approx \pm \xi^{(1)}$, we will only able to eliminate the $A^l$ component of \eqref{eq:theStressTerm}.   

We begin by expanding the low frequency part of the interactions in line \eqref{eq:theStressTerm} as
\ali{
\Th_+ U_-^l + \Th_- U_+^l &= \sum_{I, J \in \II_+} \th_I \bar{\th}_J(m^l(- \xi^{(1)}) + m^l(\xi^{(1)})) + \tx{Lower Order Terms} \label{eqref:mainNonlinearTerm} \\
&= \left| \sum_{I \in \II_+} \th_I \right|^2 A^l + \tx{Lower Order Terms} \label{eq:mainPartIsLikeAl}
}
We will give a complete list of the lower order terms below after we have chosen the amplitudes $\th_I$.

We wish to choose the amplitudes $\th_I$ so that the main term in \eqref{eq:mainPartIsLikeAl} cancels with the $A^l$ component of the other terms in line \eqref{eq:theStressTerm}.  We achieve this cancellation in two steps.  First, we decompose $R_\ep$ into components
\ali{
R_\ep^l &= c_J A^l + c_B B^l \label{eq:decomposeRepComponents}
}
We also subtract a constant vector field $\pr_l( e(t) A^l) = 0$ to line Equation \eqref{eq:theStressTerm}, leading to an equation
\ali{
\left| \sum_{I \in \II_+} \th_I \right|^2 A^l &= e(t) A^l + \tilde{c}_A A^l + c_J A^l  \\
&= e(t)(1 + \varep) A^l \label{eq:eqForThIs}\\
\varep &= \fr{\tilde{c}_A + c_J}{e(t)} \label{eq:varepTerm}
}
for the amplitudes $\th_I$.  We have assumed a lower bound \eqref{eq:lowBoundEoftx} which guarantees an upper bound of 
\[  \co{\varep} \leq \fr{Z}{K}  \]
on the size of the term \eqref{eq:varepTerm}, where $Z$ is a constant depending only on the vectors $A^l$ and $B^l$.  Then provided $K \geq K_0 = 2 Z$, we have
\ali{
\co{\varep} &\leq \fr{1}{2} \label{eq:whichK0weneed}
}

From Equation \eqref{eq:eqForThIs}, we are led to choose amplitudes of the form
\ali{
\th_I &= e^{1/2}(t) \eta_k(t) \ga, \qquad I = (k,f) \label{eq:formForThi} \\
\ga &= (1 + \varep)^{1/2}
}
The functions
\[ \eta_k(t) = \eta\left( \fr{t - k \tau}{\tau} \right) \]
are elements of a rescaled partition of unity in time
\[ \sum_{u \in \Z} \eta(t - u) = 1 \]
which we use to patch together local solutions of Equation \eqref{eq:eqForThIs}.  Our choice of $\eta_k$ ensures that each amplitude $\th_{(k,f)}$ has support in a time interval $[k \tau - \fr{2 \tau}{3},k \tau + \fr{2 \tau}{3}]$ of size $\fr{4 \tau}{3}$.  We note that our amplitudes are different from the case of the Euler equations, where one uses a partition of unity that is quadratic in nature.  The coefficients $\ga_I$ ensure that \eqref{eq:eqForThIs} is satisfied, and are assured to be well-defined by the bound \eqref{eq:whichK0weneed}.

To obtain a complete list of the lower order terms in Equation \eqref{eqref:mainNonlinearTerm}, we introduce the notation
\[ \Th_I = e^{i \la \xi_I}(\th_I + \de \th_I) = e^{i \la \xi^{(1)}\cdot x} \phi_I {\tilde \th}_I \qquad I \in \II_+ \]
where $\tilde{\th}_I = \th_I + \de \th_I$ is the corrected amplitude, and $\phi_I = e^{i \la ( \xi_I - (\pm \xi^{(1)}))}$ is a modulation factor which accounts for the difference between the phase and its initial value.  Similarly, we write
\[ U_I^l = e^{i \la \xi_I}(u_I + \de u_I) = e^{\pm i \la \xi^{(1)}\cdot x} \phi_I {\tilde u}_I^l \]
with $\tilde{u}_I^l = u_I^l + \de u_I^l$.

Using the above notation, the interaction terms from waves of opposing frequencies can be written as
\[ \Th_I {\bar U}_J^l + \bar{\Th}_I U_J^l = \phi_I \bar{\phi}_J(\tilde{\th}_I \bar{\tilde{u}}_J^l + \bar{{\tilde \th}}_I{\tilde u}_J^l), \qquad I, J \in \II_+\]
and the Lower Order Terms in \eqref{eqref:mainNonlinearTerm} are given by
\ali{
\tx{Lower Order Terms} &= R_S^l + R_{S'}^l \\
R_S^l &=  \sum_{I, J \in \II_+ } (\de \th_I \bar{{\tilde u}}_J^l + \overline{\de \th}_I {\tilde u}_J^l) \label{eq:stressError1} \\
&+ \sum_{I, J \in \II_+ } ({\tilde \th}_I \overline{ \de u}_J^l +  \bar{{\tilde \th}}_I \de u_J^l) \notag \\
&- \sum_{I, J \in \II_+ } ( \de \th_I \overline{ \de u}_J^l + \overline{\de \th}_I {\tilde u}_J^l)  \\
R_{S'}^l &= \sum_{I, J \in \II_+ } (1 - \phi_I \bar{\phi}_J)({\tilde \th}_I \bar{{\tilde u}}_J^l + \bar{{\tilde \th}}_I {\tilde u}_J^l ) \label{eq:stressError2} \\
&+ \sum_{I, J \in \II_+ } \th_I {\bar \th}_J[ (m^l(\nab \xi_I) - m^l(\xi^{(1)})) + (m^l(- \nab \xi_I) - m^l(-\xi^{(1)}))] \label{eq:stressErrorPrime}
}
The term $R_S^l$ will be small after $\la$ has been chosen sufficiently large, whereas the term $R_{S'}^l$ will be small after the lifespan parameter $\tau$ has been chosen sufficiently small.

\subsection{ The remaining error terms }

In Sections \ref{sec:shapeOfCorrections}-\ref{sec:chooseAmplitudes} we have defined the construction up to the specification of a few parameters.  Our result is that the corrected field $\th_1 = \th + \Th$ and drift velocity $u_1^l = u^l + U^l$ satisfy Equation \eqref{eq:scalarStressB} with $c_B$ defined in line \eqref{eq:decomposeRepComponents}, and
\ali{
 R_1 &= R_T + R_L + R_H + R_M + R_S + R_{S'} \label{eq:allTheErrors}
}
The terms $R_M$, $R_S$ and $R_{S'}$ are defined in \eqref{eq:mollifyRappears} and \eqref{eq:stressError1}-\eqref{eq:stressErrorPrime}.  We now rewrite the remaining terms in Equations \eqref{eq:transAndHighLow}-\eqref{eq:highFreqTerms} using the fact that the velocity fields appearing in these equations are divergence free.

The {\bf transport term} $R_T$ is obtained by solving
\ali{
\pr_l R_T^l &= (\pr_t + u_\ep^l \pr_l) \Th \label{eq:transportTerm} \\
&= \sum_I e^{i \la \xi_I} (\pr_t + u_\ep^l \pr_l){\tilde \th}_I \label{eq:explicitTransport}
}
Here the term where the derivative hits the phase functions vanishes according to equation \eqref{eq:transportEqn}.  Formula \eqref{eq:explicitTransport} suggests that the transport term has frequency $\la$, so we expect to gain a factor $\la^{-1}$ in solving equation \eqref{eq:transportTerm}.  In fact, we will choose our mollification $u_\ep$ to be a frequency-localized version of $u$ so that together with \eqref{eq:ThIisLike}, the term \eqref{eq:transportTerm} is literally supported on frequencies of size $\fr{\la}{3} \leq |\xi| \leq 2 \la$.  Hence, there is a frequency localizing operator $P_{\approx \la}$ satisfying
\[ (\pr_t + u_\ep^l \pr_l) \Th = P_{\approx \la}[ (\pr_t + u_\ep \cdot \nab) \Th ]  \]
This frequency localization property allows us to simply define
\ali{
R_T^l &= \pr^l \De^{-1} P_{\approx \la} [ (\pr_t + u_\ep \cdot \nab) \Th ]
}
In particular, we trivially obtain the bound
\ali{
 \co{R_T} &\leq \la^{-1} \co{(\pr_t + u_\ep \cdot \nab) \Th} \label{eq:transportBound1}
}

The terms remaining from \eqref{eq:transAndHighLow} and \eqref{eq:highFreqTerms} are the {\bf High-Low term}
\ali{
\pr_l R_L^l &= U^l \pr_l \th_\ep \\
&= \sum_I e^{i \la \xi_I} {\tilde u}_I^j \pr_j \th_\ep
}
and the {\bf high frequency interference terms} 
\ali{
\pr_l R_H^l &= U_-^l \pr_l \Th_- + U_+^l \pr_l \Th_+ 
}
We use frequency cutoffs in our definitions of $\th_\ep, U_\pm$ and $\Th_\pm$ so that both of these terms have Fourier support in frequencies $\fr{\la}{3} \leq |\xi| \leq 4 \la$.  Here it is important that we have localized the frequency support $\Th_I$ to a limited range of angles.  As a consequence, 
\[ U^l \pr_l \th_\ep = P_{\approx \la} [ U^l \pr_l \th_\ep ] \] 
\[ U_-^l \pr_l \Th_- + U_+^l \pr_l \Th_+  = P_{\approx \la} [U_-^l \pr_l \Th_- + U_+^l \pr_l \Th_+ ] \]
for some frequency projection operator $P_{\approx \la}$, and we can define
\ali{
R_L^l &= \pr^l \De^{-1} P_{\approx \la} [ U^j \pr_j \th_\ep ] \\
R_H^l &= \pr^l \De^{-1} P_{\approx \la} [U_-^j \pr_j \Th_- + U_+^j \pr_j \Th_+ ]
}
Now that we have written down the error terms \eqref{eq:allTheErrors}, we must observe that each of these terms can be made small.  For the transport term $R_T^l$, the estimate \eqref{eq:transportBound1} ensures that $R_T$ is small once $\la$ is chosen sufficiently large, and the same type of estimate can be used to control the High-Low term $R_L$.  The high-frequency interference terms require a more careful treatment.

Let us focus on the interference terms coming from $+, +$ interactions.
\ali{
U_+^l \pr_l \Th_+ &=  \sum_{I, J \in \II_+} ( i \la) M_{IJ} \\
&+ \sum_{I,J \in \II_+} e^{i \la(\xi_I + \xi_J)} \tilde{u}_I^l \pr_l {\tilde \th}_J \\
M_{IJ} &= e^{i \la(\xi_I + \xi_J)} \tilde{u}_I^l \pr_l \xi_J {\tilde \th}_J \label{eq:mainHighFreq1}
}
The main term $M_{IJ}$ can be expanded as
\ali{
M_{IJ} &=  e^{i \la(\xi_I + \xi_J)} (\th_I m^l(\nab \xi_I) + \de u_I^l) \pr_l \xi_J {\tilde \th}_J \\
&= e^{i \la (\xi_I + \xi_J)} ( \th_I m^l(\xi^{(1)}) \xi^{(1)}_l ) {\tilde \th}_J + \tx{Lower order terms} \label{eq:mainInterferenceTerm}
} 
The main term in \eqref{eq:mainInterferenceTerm} is actually $0$ from $m(\xi) \cdot \xi = 0$, so that only the Lower order terms contribute
\ali{
M_{IJ} &= e^{i \la (\xi_I + \xi_J)} \th_I {\tilde \th}_J ( m^l(\nab \xi_I) - m^l(\xi^{(1)}) ) \pr_l \xi_J \label{eq:MIJfirst} \\
&+ e^{i \la (\xi_I + \xi_J)} \th_I {\tilde \th}_J m^l(\xi^{(1)})( \pr_l \xi_J - \xi^{(1)}_l) \label{eq:MIJfirst2} \\
&+ e^{i \la (\xi_I + \xi_J)} \de u_I^l \pr_l \xi_J {\tilde \th}_J \label{eq:MIJlast}
}
The terms \eqref{eq:MIJfirst}, \eqref{eq:MIJfirst2} are made small by choosing the lifespan parameter $\tau$ to be small, while the term \eqref{eq:MIJlast} is made small once $\la$ is chosen sufficiently large.  The $-,-$ interaction terms are treated similarly, and the high-frequency term $R_H$ itself is then controlled by the estimate
\[ \co{R_H} \leq \fr{C}{\la} \co{U_-^j \pr_j \Th_- + U_+^j \pr_j \Th_+} \]
This calculation concludes out list of the error terms \eqref{eq:allTheErrors}.  What remains is to specify the parameters in the construction, prove estimates for the elements of the construction and finally to check that the estimates stated in Lemma \ref{lem:mainLemma} are satisfied.
